On Limited-Memory Subsampling Strategies for Bandits

There has been a recent surge of interest in nonparametric bandit algorithms based on subsampling. One drawback however of these approaches is the additional complexity required by random subsampling and the storage of the full history of rewards. Our first contribution is to show that a simple deterministic subsampling rule, proposed in the recent work of Baudry et al. (2020) under the name of ''last-block subsampling'', is asymptotically optimal in one-parameter exponential families. In addition, we prove that these guarantees also hold when limiting the algorithm memory to a polylogarithmic function of the time horizon. These findings open up new perspectives, in particular for non-stationary scenarios in which the arm distributions evolve over time. We propose a variant of the algorithm in which only the most recent observations are used for subsampling, achieving optimal regret guarantees under the assumption of a known number of abrupt changes. Extensive numerical simulations highlight the merits of this approach, particularly when the changes are not only affecting the means of the rewards.

==> algo.tex <==
\section{Algorithms}\label{sec::algos}

Dans cette partie on peut:

\begin{itemize}
	\item State les algorithmes
	\item Parler de la forced exploration
	\item Avoir la discussion sur le leader
	\item Motiver les histoires de mémoire/temps de calcul et pourqoi c'est cool par rapport aux autres SDA avec la table dont Yo parlait
\end{itemize}

\begin{algorithm}
\caption{LB-SDA}
\label{alg:lb-sda}
  \begin{algorithmic}
    \STATE{ \bfseries Input.} $K$ arms, horizon $T$, $B(r)$ forced exploration rate
    \STATE {\bfseries Initialization.}
    $t \leftarrow 1$, $r=1$ $\forall k \in \{1, ..., K \}, N_k \leftarrow 0$
    \WHILE{$t < T$}
    \STATE $\mathcal{A} \leftarrow \{\}$,
    $l \leftarrow \text{leader}(N,  t)$ %\mathcal{H})$
    \IF{$r=1$}
    \STATE $\cA \leftarrow \{1, \dots, K\}$ (Draw each arm once)
    \ELSE
    \FOR{$k \neq l \in \{1,...,K\}$}
	\IF{$N_{k} \leq B(r)$ \OR $\bar Y_{k} > \bar Y_{l, N_l- N_{k}: N_l}$   }	    	\STATE $\mathcal{A} \leftarrow \mathcal{A} \cup \{ k \}$
	\ENDIF

    	\IF{$| \mathcal{A} | = 0$}
    	\STATE $\mathcal{A} \leftarrow \{l \}$
    	\ENDIF
    \ENDFOR
    \ENDIF
    %\IF{ $|\mathcal{A}| > 1$}
%    \STATE $a \leftarrow \text{random}(\mathcal{A})$ \;\;(random element in $\mathcal{A}$)
	%\ELSE
%	\STATE $a \leftarrow \mathcal{A}$
  %  \ENDIF
  \FOR{$a \in\mathcal{A}$}
  \STATE Pull arm $a$, observe reward $Y_{a,N_a +1}$, $N_a \leftarrow N_a + 1$, $t \leftarrow t+1$
  \ENDFOR
    %$\mathcal{H}_a \leftarrow \mathcal{H}_a \cup \{Y_{a, N_a} \} $
  %  \FOR{$ k = 1,...,K$}
   % \STATE Update $N_{k, \tau}$, $t \leftarrow t+1$
    %\ENDFOR
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}


\begin{algorithm}[hbtp]
  \label{alg:DLinUCB}
\SetKwInput{KwData}{Input}
\KwData{Probability $\delta$, subgaussianity constant $\sigma$, dimension $d$, regularization $\lambda$, 
upper bound for actions $L$, upper bound for parameters $S$, discount factor $\gamma$.}
\SetKwInput{KwResult}{Initialization}
\KwResult{$b = 0_{\mathbb{R}^d}$, $V = \lambda I_d$, $\widetilde{V} = \lambda I_d$, $\hat{\theta} = 0_{\mathbb{R}^d}$}
\For{$t \geq 1$}{
Receive $\mathcal{A}_t$, compute $\beta_{t-1} = \sqrt{\lambda}S + \sigma \sqrt{2\log\left(\frac{1}{\delta}\right)+ d\log\left(1+
 \frac{L^2 (1-\gamma^{2(t-1)})}{\lambda d (1-\gamma^2) }\right)}$ \\
\For{$a \in \mathcal{A}_t$}{
Compute $\textnormal{UCB}(a) = a^{\top}\hat{\theta} + \beta_{t-1}  \sqrt{a^{\top} V^{-1} \widetilde{V} V^{-1} a} $
}
$A_t = \argmax_{a}(\textnormal{UCB}(a))$ \\
\textbf{Play action} $A_t$  and \textbf{receive reward} $X_t$ \\
\textbf{Updating phase}:
$V = \gamma V +  A_t A_t^{\top} + (1- \gamma) \lambda I_d$, $\widetilde{V} = \gamma^2 \widetilde{V} + A_t A_t^{\top} + (1-\gamma^2) \lambda I_d$ \\
$ \hspace{2.6cm} b = \gamma b + X_t A_t$, $\hat{\theta} =V^{-1}b$
}
\caption{$\DLinUCB$}
\end{algorithm}


\begin{algorithm}
\caption{LB-SDA}
  \begin{algorithmic}
    \STATE{ \bfseries Input.} $K$ arms, horizon $T$, $B(r)$ forced exploration rate
    \STATE {\bfseries Initialization.}
    $t \leftarrow 1$, $r=1$ $\forall k \in \{1, ..., K \}, N_k \leftarrow 0$
    \WHILE{$t < T$}
    \STATE $\mathcal{A} \leftarrow \{\}$,
    $l \leftarrow \text{leader}(N,  t)$ %\mathcal{H})$
    \IF{$r=1$}
    \STATE $\cA \leftarrow \{1, \dots, K\}$ (Draw each arm once)
    \ELSE
    \FOR{$k \neq l \in \{1,...,K\}$}
	\IF{$N_{k} \leq B(r)$ \OR $\bar Y_{k} > \bar Y_{l, N_l- N_{k}: N_l}$   }	    	\STATE $\mathcal{A} \leftarrow \mathcal{A} \cup \{ k \}$
	\ENDIF

    	\IF{$| \mathcal{A} | = 0$}
    	\STATE $\mathcal{A} \leftarrow \{l \}$
    	\ENDIF
    \ENDFOR
    \ENDIF
    %\IF{ $|\mathcal{A}| > 1$}
%    \STATE $a \leftarrow \text{random}(\mathcal{A})$ \;\;(random element in $\mathcal{A}$)
	%\ELSE
%	\STATE $a \leftarrow \mathcal{A}$
  %  \ENDIF
  \FOR{$a \in\mathcal{A}$}
  \STATE Pull arm $a$, observe reward $Y_{a,N_a +1}$, $N_a \leftarrow N_a + 1$, $t \leftarrow t+1$
  \ENDFOR
    %$\mathcal{H}_a \leftarrow \mathcal{H}_a \cup \{Y_{a, N_a} \} $
  %  \FOR{$ k = 1,...,K$}
   % \STATE Update $N_{k, \tau}$, $t \leftarrow t+1$
    %\ENDFOR
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{SW-LB round}
	
	\begin{algorithmic}
		\STATE{ \bfseries Input.} \begin{itemize}
			\item round $r$, leader $\ell$, challenger $k$, forced exploration rate $B(\tau)$, diversity flag $X_r^k$ 
			\item $N_k(r), N_\ell(r)$ number of pulls of the two arms since the first round, $N_{k}(r, \tau), N_{\ell}(r, \tau)$ number of pulls of the two arms during the last $\tau$ rounds.
		\end{itemize} 
		\IF{$N_k(r, \tau) < B(\tau)$ \OR $X^k=1$}
		\STATE Return $k$
		\ELSE	
		\STATE $\widehat \mu_k(r, \tau)= \bar Y_{N_k(r)-N_{k}(r, \tau)+1: N_k(r)}$ (Index of arm $k$)
		\STATE $N=\min(N_k(r, \tau), N_\ell(r, \tau))$
		\STATE $\widehat \mu_\ell^k(r, \tau)=\bar Y_{N_\ell(r)-N+1: N_\ell(r)}$ (Index of $\ell$ against $k$)
		\IF{$ \widehat \mu_k(r, \tau) \geq \widehat \mu_\ell^k(r, \tau)$}
		\STATE Return $k$
		\ENDIF
		\ENDIF
	\end{algorithmic}
\end{algorithm}


==> opt_lbsda.tex <==
\section{LB-SDA in Stationary Environments}
In this section we give some details on our subsampling strategy,
the regret guarantees for Algorithm~\ref{alg:lb-sda} and for its variant
defined in section~\ref{subsection:lb_sda_memory}.

\subsection{Last Block Sampling}
The specificity of the LB-SDA is its duel structure. Compared to the algorithms analyzed in \cite{baudry2020sub} where the sampler
is random here we consider a \textit{deterministic sampler}.
At round $r$, the duel between arm $k \neq \ell(r)$ and the leader consists in comparing the averaged reward from arm $k$ with
the average reward of the last $N_k(r)$ observations from the leader. The challenger $k$ wins its duel if
\begin{equation}
\label{eq:winning_duel_stat}
\bar Y_k \geq \bar Y_{\ell(r), N_{\ell(r)}(r) - N_k(r) + 1 : N_{\ell(r)}(r)} \;.
\end{equation}
To enforce some diversity in the duels, we also draw the arms  for which the number of pulls in under a fixed threshold denoted $B(r)$.
If the leader wins \textit{all} its duel then it is drawn, otherwise all the winning challengers and the under-explored arms are pulled.
The algorithm is reported in Algorithm \ref{alg:lb-sda}.
% The intuition is that by subsampling a portion of the history of the leader we introduce a natural form of exploration. Yet, it is quite surprising

\begin{algorithm}[hbtp]
\SetKwInput{KwData}{Input}
\KwData{$K$ arms, horizon $T$, $f(r)$ forced exploration rate}
\SetKwInput{KwResult}{Initialization}
\KwResult{$t \leftarrow 1$, $r=1$ $\forall k \in \{1, ..., K \}, N_k \leftarrow 0$}
\While{$t < T$}{
$\mathcal{A} \leftarrow \{\}$,  $\ell \leftarrow \text{leader}(N,  t)$ \\
\If{$r=1$}{
$\cA \leftarrow \{1, \dots, K\}$ (Draw each arm once)}
\Else{
\For{$k \neq \ell \in \{1,...,K\}$}{
\If{$N_{k} \leq f(r)$ \text{or} $\bar Y_{k} > \bar Y_{\ell, N_{\ell}- N_{k}: N_{\ell} }$ }{$\mathcal{A} \leftarrow \mathcal{A} \cup \{ k \}$}
\If{$| \mathcal{A} | = 0$}{$\mathcal{A} \leftarrow \{l \}$}
}
}
\For{$a \in \mathcal{A}$}{
Pull arm $a$, observe reward $Y_{a,N_a +1}$, $N_a \leftarrow N_a + 1$, $t \leftarrow t+1$
}
}
\caption{LB-SDA}
\label{alg:lb-sda}
\end{algorithm}

\subsection{Regret analysis of LB-SDA}
\label{subsection:lb_sda_stat}
We consider that the arms come from the same 1-parameter exponential family of distributions
$\cP_{\Theta}$, i.e there exists a function $g: \R \times \Theta \mapsto \R$
such that any arm $k$ has a density of the form \[g_k(x) = g(x, \theta_k) = e^{\theta_k x - \Psi(\theta_k)} g(x, 0) \;,\]

where $\Psi(\theta_k) = \log \left[\int e^{\theta_k x} g(x, 0) \,dx\right]$.
This assumption is standard in the literature and covers a broad range of bandits applications.%many applications of
%bandit algorithms.
The exact knowledge of the family of distributions
of the arms (e.g Bernoulli, Gaussian, Poisson, etc.) can ensure proper
calibration of algorithms like Thompson Sampling \cite{TS_Emilie}, KL-UCB \cite{cappe2013kullback} or IMED
 \cite{Honda15IMED} to reach asymptotic optimality.
 Recently, subsampling algorithms like SSMC \cite{chan2020multi} and
 RB-SDA \cite{baudry2020sub} have been proved to be optimal \textit{without}
 knowing exactly $\cP_\Theta$. This means that the exact same algorithm
 can be run on Bernoulli,
 Gaussian or Poisson distributions (which are all exponential families)
 and still achieve optimality.
 Our first contribution consists in proving that LB-SDA
 matches the theoretical guarantees of existing subsampling algorithms.

\begin{theorem}
\label{th::regret_lbsda}
	For any bandit model $\nu=(\nu_1, \dots, \nu_K) \subset \cP_{\Theta}^K$ where $\cP_\Theta$ is any 1-parameter exponential family of distributions, the regret of LB-SDA satisfies for all $\epsilon >0$
	$$
	\cR(T) \leq \sum_{k: \mu_k < \mu^\star} \frac{1+\epsilon}{\kl(\mu^\star, \mu_k)} \log(T) + C(\nu, \epsilon) \;.
	$$
\end{theorem}

%To prove this result we build on Lemma 4.1 of \citet{baudry2020sub},
%\todoyo{est-ce que ça ne vaudrait pas mieux de partir de chan pour ici ? de plus dans le statement de 4.1 dans le papier nips tu dis que la différence avec chan c'est l'absence de forced exploration, étant donné qu'on a la forced exploration ici,on doit être plus proche de chan j'imagine.}
We assume without loss of generality that there is a unique optimal arm denoted $k^\star$.
Using the analysis of \citet{chan2020multi} and \citet{baudry2020sub} for any SDA algorithm the number of pulls of a suboptimal at a time horizon $T$.

\begin{lemma}[Lemma 4.1 in \cite{baudry2020sub}]
\label{lem::dec_statio}
	For any suboptimal arm $k \neq k^\star$ the expected number of pulls of $k$ is upper bounded by
	 \begin{equation}
	\begin{split}
	\bE[N_k(T)] &\leq \frac{1+\epsilon}{\kl(\mu^\star, \mu_k)} \log(T) + C_k(\nu, \epsilon) \\
	&+ 32 \sum_{r=1}^T \bP(N_{k^\star}(r)\leq (\log r)^2)\;,
	\end{split}
	\end{equation}
	where $C_k(\nu, \epsilon)$ is a problem-dependent constant.
\end{lemma}

%Lemma \ref{lem::dec_statio} do not use the specificity of the sampler and
The decomposition from Lemma \ref{lem::dec_statio} is valid for any SDA algorithm.
%Using Lemma \ref{lem::dec_statio} it remains
%Thanks to this result the analysis is reduced
The next step consists in upper bounding the probability that the best arm is not pulled "enough" during a run of the algorithm.
This part is more challenging and relies on a notion of \textit{diversity} in the subsamples provided by the subsampling algorithms
in RB-SDA \cite{baudry2020sub}. %However, in RB-SDA a random block is sampled at each reach round
Unfortunately, this property is not satisfied by deterministic samplers as such Last-Block.
When it was intuitive that the Random Block sampler will
explore different part of the history thus bringing diversity in the duels,
it is quite surprising that similar guarantees can be obtained when only considering the last block.
%It comes at no surprise that adding some forced exploration is required to obtain diverse duels
%the analysis of RB-SDA in \citet{baudry2020sub} and heavily relies on a notion o that is not satisfied by deterministic algorithms like the Last-Block sampler.
However, combining some inherent properties of Last-Block sampling with some well tuned forced exploration is sufficient in
order to prove that the number of pulls of the optimal arm is large enough with high probability for LB-SDA too.

\begin{lemma}
\label{lem::control_pull_lbsda_s}
\[\sum_{r=1}^T \bP\left(N_{k^\star}(r) \leq (\log r)^2\right) \leq C_{k^\star}(\nu, \epsilon) \;,\]
for some constant $C_1(\nu, \epsilon)$.
\end{lemma}

\begin{proof}
	The proof of this result is reported in Appendix~\ref{app::proof_s}.
\end{proof}

%\tododo{A partir de là deux possibilités: sont on rentre dans les détails du sketch en remettant la balance condition, la diversité etc, sont on décrit de manière globale ce qu'il se passe, on highlight la contrib et on pointe vers les appendix. ça me parait raisonnable de s'arrêter là et de passer à la memory direct.}

\subsection{Memory-limited LB-SDA}
\label{subsection:lb_sda_memory}
One of our main motivations for studying LB-SDA is its simplicity and efficiency. Yet, all existing subsampling algorithms
\cite{baudry2020sub, chan2020multi} as well as the vanilla version of LB-SDA
have to store the entire reward's history for the different arms.
%Reducing the storage while maintaining the theoretical guarantees is of interest for large time horizons.
In this section, we explain how to modify LB-SDA to reduce the storage while preserving the theoretical guarantees.

%One of the main motivations of our study of LB-SDA is the simplicity and efficiency of LB-SDA. However, the vanilla LB-SDA shares with the other efficient bandit algorithms based on subsampling (SSMC, RB-SDA) the drawback that they require to store the full history of rewards, which cost $T$ for any time horizon $T$. This can become an issue, in particular when $T$ is large.


%However, intuitively when $T$ is large and after the optimal arm $1$ becomes leader and the other arms all have a number of pull in $O(\log T)$ the definition of Last Block sampling will ensure that we will \textit{never} use the first observations of arm $1$ again. We can even add that only $O(\log T)$ observations will actually be used by the algorithm. Unfortunately, it is impossible to reduce the storage requirements of the algorithm to this quantity because the optimal tuning would require the knowledge of the gaps.

Knowing that LB-SDA is asymptotically optimal, when $T$ is large the arm with the largest mean necessarily
becomes the leader and all its challenger should have a number of pull $O(\log T)$. With duels based on the Last Block, this would mean
in particular that only the last $O(\log T)$ observations of the optimal arm should be used and previous observations will \textit{never} be used.
Based on this intuition,
one might think that keeping only $\log(T)/(\mu^\star- \mu_k)$ observations is enough for LB-SDA.  Yet, this can only be done
with the knowledge of the gaps that are unknown.



We propose instead to limit the storage memory of each arm at a round
$r$ to a value $m_r = \max\left(M, \left\lceil C(\log r)^2\right\rceil\right)$,
for some constants $M \in \N$ that could represent a minimum number of samples
we are ready to collect for each arm and $C>0$.
The idea of the constant $M$ is to avoid slowing down the learning
on the beginning of a trajectory when the number of samples is small.
We then define the set of saturated arms at a round $r$ as
$$\cS_r = \{k \in \K: N_k(r)\geq m_r\} \;.$$
The only modification of the LB-SDA is the following:
 at each round $r$, if a saturated arm is pulled then the newly collected observation replaces the oldest observation in its history.
 Our second contribution in stationary environments is the proof that LB-SDA keeps its asymptotical guarantees
  under the memory limited setting. The statement of LB-SDA-LM (Last Block Sampling Duelling
  algorithm with Limited Memory) is reported in Appendix \ref{}.

\begin{theorem}
	For any bandit model $\nu=(\nu_1, \dots, \nu_K) \subset \cP_{\Theta}^K$
	where $\cP_\Theta$ is any 1-parameter exponential family of distributions.
	If we define a sequence $m_r=\max\left(M, \left\lceil C(\log r)^2\right\rceil\right)$
	for some constants $M \in \N$ and $C>0$, the regret of the corresponding memory-limited LB-SDA
	satisfies for all $\epsilon >0$
	\[\cR_T \leq \sum_{k=2}^K \frac{1+\epsilon}{\kl(\mu_1, \mu_k)} \log(T) + C'(\nu, \epsilon, \cM) \;,\]
	where $\cM=(m_1, m_2, \dots, m_T)$ is the full infinite sequence $(m_r)_{r \in \N}$.
\end{theorem}

\begin{proof} Building on the original proof of
Theorem~\ref{th::regret_lbsda} in \citet{baudry2020sub} we provide a complete proof of the theorem in Appendix~\ref{app::proof_4.1}.
\end{proof}
We had to rewrite most of the events to take in account the memory limitation
and we tried to clearly exhibit the new terms and their dependence in $m_r$.
In practice, the smallest the constants $C$ and $M$ the largest the constant $C(\nu, \epsilon, \cM)$ will be.
Hence a trade-off between the algorithm performance and its memory consumption.
%For the practitioners, there is a new trade-off between the memory
%and the performance gain of larger storage capacities.
%Hence, there is a trade-off for practitioners between the memory resource
%they are ready to allow for the algorithm to use and the performance gain of larger storage capacities.

\begin{table}[t]
\caption{Sampling rule and storage for existing subsampling algorithm.}
\label{tab:samp}
\vskip 0.15in
\begin{center}
\begin{small}
%\begin{sc}
\begin{tabular}{ccc}
\toprule
Algorithm & Storage & Sampling\\
\midrule
\begin{tabular}{c} SSMC \\
         \cite{chan2020multi}\end{tabular}
          & $O(T)$ & Deterministic \\
          \midrule
 \begin{tabular}{c} RB-SDA \\ \cite{baudry2020sub}\end{tabular}
       & $O(T)$ & Random \\
       \midrule
\begin{tabular}{c} LB-SDA \\ \textbf{(this paper)} \end{tabular}
& $O(T)$ & Deterministic\\
\midrule
\begin{tabular}{c} LB-SDA-LM \\ \textbf{(this paper)} \end{tabular} &  {\color{red} $O(\log(T)^2)$}
& Deterministic         \\
\bottomrule
\end{tabular}
%\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> proof_lbsda_old.tex <==
\section{Proof of Theorem~\ref{th::log_regret_sda}}\label{app::proof_4.1}

\subsection{Notation for the Proof}\label{app::notations}
	

General notations for the stationary case:
\begin{itemize}
	\item $K$ number of arms
	\item $\nu_k$ distribution of the arm $k$, with mean $\mu_k$
	\item we assume that $\mu_1 = \max_{k \in [K]} \mu_k$ so we call the (unique) optimal arm "arm 1"
	\item $I_k(x)$ some rate function of the arm $k$, evaluated in $x$. For 1-parameter exponential families this function will always be the KL-divergence between $\nu_k$ and the distribution from the same family with mean $x$.
	\item $N_k(r)$ number of pull of arm $k$ up to (and including) round $r$.
	\item $Y_{k, i}$ reward obtained at the i-th pull of arm $k$.
	\item $\hat Y_{k, i}$ mean of the i-th first reward of arm $k$, $\hat Y_{k, n:m}$ mean of the rewards of $k$ on a subset of indices $[n:m]$, $n<m$:  $\hat Y_{k, n:m}= \frac{1}{m-n} \sum_{i=n}^m Y_{k, i}$. If $m-n=s$, then $Y_{k, s}$ and $Y_{k, n:m}$ have the same distribution.
	\item $\ell(r)$ leader at round $r+1$, $\ell(r)=\text{argmax}_{k \in [K]} N_k(r)$.
	\item $(S_k^r(m, n))_{m \geq n}$ a family of independent random variables such that $S_k^r(m, n) \sim \text{SP}(m, n, r)$. 
	\item $\cA_r$ set of arms pulled at a round $r$.
	\item $\mathcal{R}_r$ regret at the \textit{end} of round $r$.
\end{itemize}

Notations for the regret analysis, part relying on concentration:
\begin{itemize}
	\item $\cG_k^T = \cup_{r=1}^{T-1} \{\ell(r)=1\} \cap  \{k \in \mathcal{A}_{r+1}\} \cap \{N_k(r) \geq (1+\epsilon) \xi_k \log T\}$ 
	
	\item $\cH_k^T = \cup_{r=1}^{T-1} \{\ell(r)=1\} \cap  \{k \in \mathcal{A}_{r+1}\} \cap \{N_k(r) \geq J_k \log T\}$ 
	
	\item $\cZ^r = \{\ell(r) \neq 1\}$, the leader used at round  $r+1$ is sub-optimal.
	
	\item $\cD^r = \{\exists u \in  [\lfloor r/4 \rfloor, r] \text{ such that } \ell(u-1) = 1 \}$, the leader has been optimal at least once between $\lfloor r/4 \rfloor$ and $r$
	\item $\cB^{u} = \{\ell(u)=1, k \in \mathcal{A}_{u+1}, N_k(u)=N_1(u)-1 \text{ for some arm } k \}$, the optimal arm is leader in $u$ but loses its duel again some arm $k$, that have been pulled enough to possibly take over the leadership at next round
	\item $\cC^u = \{\exists k \neq 1, N_k(u)\geq N_1(u), \hat Y_{k,S_1^u(N_k(u),N_{1}(u))} \geq \hat Y_{1,N_1(u)}\}$, the optimal arm is not the leader and has lost its duel against the sub-optimal leader.
	\item $\cL^r= \sum_{u=\lfloor r/4 \rfloor}^r \ind_{\cC^u}$
\end{itemize}

	
\subsection{Part 1: Concentration}
	
The beginning of the proof of ~\citet{baudry2020sub} is valid for \LBSDA{}, but we rewrite it for the sake of completeness and to highlight the parts that have to be changed to make the theorem hold with a limited memory usage that we write $m_r = \Omega\left((\log r)^2\right)$. We assume that $m_r$ is an integer for any round $r$, and the condition takes the form that at any round $r$ the index of an arm can be computed at most on its $m_r$ last observations.

We assume that arm $1$ is the only optimal arm: $\mu_1=\max_{k \in [K]} \mu_k$. For each arm $k$ we write $x_k, \omega_k$ as the values satisfying $I_k(x_k)=I_1(x_k)=\omega_k$ for the rate functions $I_1$ and $I_k$.

For any arm $k$ we write 

\begin{align}
\mathbb{E}[N_k(T)]& = \mathbb{E}[N_k(T) \ind_{\cH_k^T}] + \mathbb{E}[N_k(T) \ind_{\cG_k^T} \ind_{\bar{\cH}_k^T}] +\mathbb{E}[N_k(T) \ind_{\bar{\cG}_k^T}]   \nonumber\\
& \leq T \mathbb{P}(\cH_k^T) + (1+J_k \log T)  \mathbb{P}(\cG_k^T) + 1 + (1+\epsilon)\xi_k \log T  + 2 \sum_{r=1}^{T-1} \mathbb{P}(\cZ^r)\label{eq:dec}
\end{align}

Indeed, due to the definition of each event we have:
\begin{align*} N_k(T) \ind_{\bar{\cG}_k^T} 
& \leq  1 + \sum_{r=1}^{T-1}\ind_{(k \in \cA_{r+1})}\ind_{(\ell(r) \neq 1)\cup(N_{k}(r) < (1+\epsilon)\xi_k \log(T))}\\
& \leq  1 + \sum_{r=1}^{T-1}\ind_{(k \in \cA_{r+1})}\ind_{(N_{k}(r) < (1+\epsilon)\xi_k \log(T))} + \sum_{r=1}^{T-1}\ind_{(\ell(r) \neq 1)}\\
& \leq  
1 + (1+\epsilon) \xi_k \log T + \sum_{r=1}^{T-1} \ind_{\cZ^r}\end{align*}
and similarly
\begin{align*}
N_k(T) \ind_{\cG_k^T} \ind_{\bar{\cH}_k^T} &\leq \left(1 + J_k \log T + \sum_{r=1}^{T-1} \ind_{\cZ^r}\right) \ind_{\cG_k^T} \\
& \leq (1 + J_k \log T) \ind_{\cG_k^T}  + \sum_{r=1}^{T-1} \ind_{\cZ^r}
\end{align*}


Choosing $\xi_k=1/I_1(\mu_k)$ the bound in~\eqref{eq:dec} exhibits the term in $\frac{1+\epsilon}{I_1(\mu_k)} \log T$ in Lemma~\ref{lem:dec}. To obtain the result, it remains to upper bound
\[ T \mathbb{P}(\cH_k^T) + (1+J_k \log T)  \mathbb{P}(\cG_k^T) +  2 \sum_{r=1}^{T-1} \mathbb{P}(\cZ^r)\]
for an appropriate choice of $J_k$. To do so, we shall first use concentration results to upper bound the terms involving $\cG_k^T$ and $\cH_k^T$ by problem-dependent constants (Appendix~\ref{app::bound_G_H}), and then we carefully handle the terms in $\cZ^r$ (Appendix~\ref{app::boundZ}).

\subsubsection{Divagations sur la memory limitation}

\tododo{Brouillon sur la memory limit}

On peut faire le choix de redéfinir le leader ou non. Ne pas redéfinir = compréhension de l'algo straightforward, on ne se "disperse" pas, Yo était plus pour ça. Redéfinir = On pousse à fond la carte de memory limited.

Si on redéfinit pas on ne change pas la preuve mais les constantes vont devenir plus dégueu un peu partout. Si on redéfinit on peut pas mal changer la preuve en utilisant notamment les props qui vont suivre. Je propose un petit sketch dans la V2.

\paragraph{Def du leader} $\ell(r)=\aargmax_{k: N_k(r)\geq m_r} \bar Y_{N_k(r)-m_r+1: N_k(r)}$. Cette fois on prend le meilleur bras empiriquement parmi ceux qui ont été assez tirés. On peut voir les duels comme un truc en deux étapes à présent: 
\begin{enumerate}
	\item Leader selection: all arms that have been drawn more than $m_r$ times and that are not the leader will not play the duels and will not be drawn
	\item Duels between the leader and the challengers (here: arms that have been played less than $m_r$ times): index of the challengers = empirical mean, index of the leader = LB, nothing change in this step.
\end{enumerate}

We can define a set $\cS_r= \{k \in \K: N_k(r) \geq m_r\}$, "saturated" arms at round $r$. This notion of saturated arms come from an article about TS from Agrawal et al. (find the ref). Main property: if an arm is saturated, either it is the leader or it is not pulled.

\paragraph{Sketch}

\begin{itemize}
\item $1 \in \cS_r, k \in \cS_r$ duels entre deux bras concentrés avec $m_r$ samples. On peut upper bounder par $2\sum_{k=2}^K \sum_{r=r_0}^T r e^{-m_r \omega_k}$. C'est un peu plus dégueu que sans memory limit mais ça converge bien.
\item $1 \in \cS_r, k \notin \cS_r$, là c'est exactement comme avant avec $\cG_k^T$ et $\cH_k^T$, car on va faire du LB-subsampling exactement pareil (le seul changement est qu'on diminue la somme sur $n_k$ mais de toute manière on borner en prenant la valeur de la somme infinie déjà avant).
\item $1 \notin \cS_r$, c'est notre $\bP(N_1(r)\leq m_r)$ d'avant mais attention on ne peux pas le gérer directement avec la diversité. En effet, $1$ pourrait avoir été saturé pendant une période puis plus du tout. Je propose un trick similaire à d'habitude: on regarde si $N_1(r) \geq m_r/4$ ou $N_1(r)\leq m_r/4$. Dans le premier cas on upper bound par la probabilité que $1$ perde en étant quand pas mal concentré (en ordre de grandeur c'est pareil que $m_r$), dans le second ça veut dire que $1$ est assez loin de la saturation: ça veut dire que ça fait très longtemps que la saturation n'a pas pu être activée sur lui: il a perdu un grand nombre de duel avec un sample fixe. En résumé on aura \begin{itemize}
	\item $1 \notin \cS_r, N_1(r) \geq m_r/4-1$: gérer comme le premier point
	\item $1 \notin \cS_r, N_1(r) \leq m_r/4-1$: ça fait un bail que $1$ a pas été saturé, on va pouvoir appliquer la diversité. Avec $m_r/4-1$ on est sûr qu'il n'est plus saturé depuis au moins $\sqrt{r}$
\end{itemize}
\end{itemize}




\subsubsection{Upper Bounds on $\bP (\cG_k^T)$ and $\bP (\cH_k^T)$}\label{app::bound_G_H}

In this part we do not consider the memory limitation, as it would be equivalent to add the conditions $N_k(r)\leq m_r$ for all $k$. We first fix for any $k\neq 1$ some real numbers $J_k, y_k$ that will be specified later, and $\xi_k=1/I_k(\mu_1)$. 
Starting with $\cG_k^T$, we write $n_0(T)=(1+\epsilon)\xi_k \log T$ and obtain

\begin{align*}
\bP (\cG_k^T) & \leq \sum_{r=1}^{T-1} \bP\left(\ell(r) = 1, k \in \cA_{r+1}, N_k(r) \geq n_0(T) \right) \\
& \leq \sum_{r=n_0(T)}^{T-1} \bP\left(N_1(r)\geq N_k(r), \bar Y_{k,N_k(r)} > \bar Y_{1, N_1(r)-N_k(r):N_1(r)}, N_k(r) \geq n_0(T), k \in \cA_{r+1} \right)\\
& \leq \sum_{r=n_0(T)}^{T-1}\bP\left(N_1(r)\geq N_k(r), \left\{\bar Y_{k,N_k(r)} \geq y_k \cup \bar Y_{1, N_1(r)-N_k(r):N_1(r)} \leq y_k \right\}, N_k(r) \geq n_0(T), k \in \cA_{r+1} \right)\\
& \leq \sum_{r=n_0(T)}^{T-1} \sum_{n_k=n_0(T)}^{T-1}  \bP\left(\bar Y_{k, n_k} \geq y_k, N_k(r)=n_k, k \in \cA_{r+1} \right) \\
& + \sum_{r=n_0(T)}^{T-1} \sum_{n_k=n_0(T)}^{T-1} \sum_{n_1=n_0(T)}^{T-1} \bP\left(\bar Y_{k, n_1-n_k:n_1} \geq y_k, N_k(r)=n_k, N_1(r)=n_1, k \in \cA_{r+1} \right) \;.\\
\end{align*}

\tododo{Attention attention, il faut séparer $N_k \leq m_r$ et $N_k \geq m_r$. En effet, au dessus de $m_r$ il faut faire un truc en mode SW donc c'est pas tout à fait pareil! On va payer un $r$ dans le 2e terme, mais ça sera pas grave asymptotiquement.}

We then use that $\sum_{r=1}^T \ind(k\in \cA_{r+1}, N_k(r)=n_k) \leq 1$ for any $n_k$ to upper bound the sum in $r$ and write

\begin{align*}
\bP\left(\cG_k^T \right)& \leq \sum_{n_k=n_0(T)}^{T-1} \bP\left(\bar Y_{k, n_k} \geq y_k\right) + \sum_{n_k=n_0(T)}^{T-1} \sum_{n_1=n_0(T)}^{T-1} \bP\left(\bar Y_{k, n_1-n_k:n_1} \leq y_k\right)\\
& \leq \sum_{n_k=n_0(T)}^{T-1} \bP\left(\bar Y_{k, n_k} \geq y_k\right) + T \sum_{n_k=n_0(T)}^{T-1} \bP\left(\bar Y_{1, n_k} \leq y_k\right)\\
&\leq \frac{T}{1-e^{-I_k(y_k)}} e^{-n_0(T)I_k(y_k)} + \frac{1}{1-e^{-I_{k}(y_k)}} e^{-n_0(T)I_k(y_k)}\;,
\end{align*}

where we also used that $\bP\left(\bar Y_{1, n_k} \leq y_k\right)=\bP\left(\bar Y_{1, n-n_k:n} \leq y_k\right)$ for any $n$. With the exact same steps we obtain
\begin{align*}
\bP (\cH_k^T) \leq \frac{T}{1-e^{-\omega_k}} e^{-J_k \omega_k \log T } + \frac{1}{1-e^{-\omega_k}} e^{-J_k\omega_k \log T}\leq (T+1)\frac{e^{-J_k\omega_k \log T}}{1-e^{-\omega_k}}\;.
\end{align*}

Our objective is to bound $T\bP(\cH_k^T)$ and $\log (T) \bP(\cG_k^T)$ by constants. This is achieved for instance if $T\bP(\cH_k^T) \underset{T\to +\infty}{\longrightarrow} 0$ and $\log (T) \bP(\cG_k^T)\underset{T\to +\infty}{\longrightarrow} 0$. The condition on $J_k$ is satisfied with for instance with $J_k = \frac{3}{\omega_k}$. On the other hand, term in $\cG_k^T$ requires $(1+\epsilon) \frac{I_k(y_k)}{I_k(\mu_1)} >1$, so we can for instance choose $y_k$ as the value satisfying $I_k(y_k)= \frac{I_k(\mu_1)}{1+\epsilon/2}$. It is possible to choose this value thanks to the continuity of the rate function.

Choosing these values, both the terms in $\cG_k^T$ and $\cH_k^T$ in \eqref{eq:dec} are part of the constant $C_{k}(\nu,\epsilon)$ in Lemma~\ref{lem:dec}. We can now focus on upper bounding $\sum_{r=1}^{T-1} \bP (\cZ^r)$, which is more challenging.

\subsubsection{Upper Bound on $\sum_{r=1}^{T-1} \bP(\cZ^r)$}\label{app::boundZ}

%The concentration inequality of Lemma \ref{concentration} allows to now restrict our analysis to the identity of the leader at all rounds. 

In a stationary environment, with an infinite storage capacity the definition of the leader ensures the following property,
\begin{align*}
\ell(r) = k \Rightarrow N_k(r) \geq \left\lceil \frac{r}{K}\right\rceil \;.
\end{align*}

However, adding the storage constraint we have that for any $r$ satisfying $r \geq K m_r$ the leader has exactly necessarily more than $m_r$ observations, so its history will be truncated to the $m_r$ last observations. If $r$ is large enough we still have good concentration guarantees for the leader after a reasonable amount of rounds, that we are going to use in this section. We define $a_r=K(m_r+1)$ and use the decomposition
\begin{equation}\bP\left(\cZ^r\right)= \bP\left(\cZ^r \cap \cD^r\right) + \bP\left(\cZ^r \cap \bar\cD^r\right),\label{dec:Z}\end{equation}
for any $r\geq r_0$ satisfying $r\geq K (m_r+1)$, where $\cD^r$ is the event that the optimal arm has been leader at least once in $[a_r,r]$: 
\[\cD^r = \{\exists u \in  [a_r, r] \text{ such that } \ell(u) = 1 \}.\]
We now explain how to upper bound the sum of the two terms in the left hand side of~\eqref{dec:Z}.

\subsubsection{Controlling $\bP(\cZ^r\cap\cD^r)$: arm 1 has been leader between $a_r$ and $r$}
\tododo{brouillon pour demain}
$\ell(s)=\best, \ell(s+1)\neq \best \Rightarrow \{\exists k, N_k(s)=N_1(u)-1, k \in \cA_{s+1}$ ET le dernier bloc de taille $m_r$ sous/sur-performe blabla.

\tododo{in brouillon}

We introduce a new event 
\begin{align*}
%\cD^s& =& \{\exists u \in  [s_0, s] \text{ such that } \ell_{u} = 1 \}\\
&\cB^{u} = \{\ell(u)=1, k \in \mathcal{A}_{u+1}, N_k(u)=N_1(u)-1 \text{ for some arm } k \}&
\end{align*}
If $\cD^r$ happens, then the event $\cZ^r$ can be true only if the leadership has been taken over by a sub-optimal arm at some round between $a_r$ and $r$, that is 
$$
\cZ^r \cap \cD^r \subset \cup_{u=a_r}^{r-1}\{\cZ_u^c, \cZ_{u+1} \} \subset \cup_{u=a_r}^{r-1} \cB^u
$$
We now upper bound $\sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \bP(\cB^u)$. We use the notation $b_r=\lceil a_r/K \rceil$ representing the minimum of samples of the leader at the round $a_r$. Hence we are sure that under $\cB^u$ arm $1$ had at least $b_r$ observations when it lost the duel that cost it the leadership. We then take an union bound on all the sub-optimal arms $k \in \K$, $\cB^u = \cup_{k=2}^K \cB_k^u := \left\{\ell(u)=1, k \in \mathcal{A}_{u+1}, N_k(u)=N_1(u)-1\right\}$, which fixes a specific suboptimal arm.
Choosing $x_k, \omega_k$ as in the previous part we can write {\small
	\begin{align}
	&\sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \bP(\cB_k^u)  = \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^{r} \ind(\ell(u)=1) \ind(k \in \cA_{u+1}) \ind(N_1(u)=N_k(u)+1) \nonumber \\ 
	& \leq \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \ind(N_1(u) \geq  b_r) \ind(\bar Y_{k, N_k(u)} \geq \bar Y_{1, N_1(u)-N_k(u):N_1(u)}) \ind(N_1(u)=N_k(u)+1) \ind(k\in \cA_{u+1}) \nonumber\\
	& \leq \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \ind(N_1(u) \geq  b_r) \ind( \bar Y_{k,N_k(u)} \geq x_k) \ind(N_1(u)=N_k(u)+1) \ind(k\in \cA_{u+1}) 
	\label{eq:FirstPart}\\ 
	& + \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \ind(N_1(u) \geq  b_r) \ind( \bar Y_{1,N_1(u)-N_k(u):N_1(u)} \leq x_k) \ind(N_1(u)=N_k(u)+1) \ind(k\in \cA_{u+1}) \;. \label{eq:SecondPart}
	\end{align}}

We now separately upper bound each of these two terms. First, 
\begin{align*}
\eqref{eq:FirstPart} & \leq  \bE\sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \sum_{n_k = b_r -1}^{r} \ind(N_k(u) = n_k) \ind(k\in \cA_{u+1})\ind( \bar Y_{k,n_k} \geq x_k) \\
& \leq  \bE\sum_{r=r_0}^{T-1}  \sum_{n_k = b_r -1}^{r} \ind( \bar Y_{k,n_k} \geq x_k) \underbrace{\sum_{u=a_r}^r\ind(N_k(u) = n_k) \ind(k\in \cA_{u+1})}_{\leq 1} \\
& \leq \sum_{r=r_0}^{T-1}  \sum_{n_k = b_r -1}^{r} \bP( \bar Y_{k,n_k} \geq x_k) \\
& \leq \sum_{r=r_0}^{T-1} \sum_{n_k = b_r -1}^{r} \exp\left(-n_k \omega_k \right)  \\
& \leq \sum_{r=r_0}^{T-1}\frac{e^{-(b_r -1) \omega_k}}{1-e^{-\omega_k}} \;. \\
\end{align*}
We remark that by definition $b_r \geq a_r/K \geq r/4K$, so we conclude that
\begin{align*}
\eqref{eq:FirstPart}& \leq \frac{e^{1- \frac{2}{K}\omega_k}}{(1-e^{-\omega_k})(1-e^{-\omega_k/4K})} \;.
\end{align*}

As the sub-sampling in LB-SDA is deterministic the relationship between $N_k$ and $N_1$ in the event we consider allow us to use the same method to upper bound \eqref{eq:SecondPart} as for \eqref{eq:FirstPart}, 

\begin{align*}
\eqref{eq:SecondPart} & \leq \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \sum_{n_k = b_r -1}^{r} \ind( \bar Y_{1,2:n_k+1} \leq x_k) \ind(N_k(u) = n_k) \ind(k\in \cA_{u+1}) \\
& \leq \bE \sum_{r=r_0}^{T-1} \sum_{u=a_r}^r \sum_{n_k = b_r -1}^{r}  \ind( \bar Y_{1,2:n_k+1} \leq x_k) \ind(N_k(u) = n_k) \ind(k\in \cA_{u+1}) \\
& \leq \bE \sum_{r=r_0}^{T-1} \sum_{n_k = b_r -1}^{r} \ind( \bar Y_{1,2:n_k+1} \leq x_k) \underbrace{\sum_{u=a_r}^r \ind(N_k(u) = n_k) \ind(k\in \cA_{u+1})}_{\leq 1} \\
& \leq \sum_{r=r_0}^{T-1} \sum_{n_k = b_r -1}^{r} \bP( \bar Y_{1, n_k} \leq x_k )\\
& \leq \frac{e^{1- \frac{2}{K}\omega_k}}{(1-e^{-\omega_k})(1-e^{-\omega_k/4K})} \;.
\end{align*}

Summing on all sub-optimal arms $k$ we finally obtain
\begin{equation}\label{eq::bound_B}
\sum_{r=r_0}^{T-1}\bP\left(\cZ^r \cap \cD^r\right) \leq \sum_{r=8}^{T-1} \sum_{u=a_r}^r \bP(\cB^u) \leq \sum_{k=2}^K  2\frac{e^{1- \frac{2}{K}\omega_k}}{(1-e^{-\omega_k})(1-e^{-\omega_k/4K})}\;.
\end{equation}

\tododo{On note que dans le 2e terme il y a un petit improvement par rapport à la preuve dans neurips où on avait un carré au dénominateur. Encore une fois, à voir si ces petits tricks sont suffisants pour que ça vaille le coup de remettre toute la preuve.}

\subsubsection{Controlling $\bP(\cZ^r\cap\cD^r)$: arm 1 has not been leader between $\lfloor r/4 \rfloor$ and $r$}

The idea in this part is to leverage the fact that if the optimal arm is not leader between $\lfloor s/4 \rfloor$ and $s$, then it has necessarily lost a lot of duels against the current leader at each round. We then use the fact that when the leader has been drawn "enough", concentration prevents this situation with large probability. We introduce
$$\cL^r= \sum_{u=s_0}^r \ind_{\cC^u}\,  $$
for the event $\cC^u= \{\exists k \neq 1, N_k(u)\geq N_1(u), \bar Y_{k,N_k(u)-N_1(u):N_k(u)} \geq \bar Y_{1,N_1(u)}\}.$ One can prove the following inequality: 
\begin{align*}
\bP(\cZ^r \cap \bar \cD^r) \leq \bP(\cL^r\geq r/4)\;. 
\end{align*}
\begin{proof} Under $\bar \cD^r$ arm $1$ is a challenger for every round  $u \in [a_r, r]$. Then, each time $\cC^u$ is not true arm 1 wins its duel against the current leader and is pulled. Hence, if $\{ \cL_r<r/4 \}$ then we necessarily have $\{N_1(r)>r/2\}$ and arm $1$ is leader in round $r$. Hence, $\{\cZ^r \cap \bar \cD^r \} \cap \{ \cL_r<r/4 \} = \emptyset$, which justifies the inequality.
\end{proof}


Now, as in \cite{chan2020multi} we use the Markov inequality to get:
\begin{align*}
\bP(\cL^r\geq r/4) \leq \frac{\bE(\cL^r)}{r/4}= \frac{4}{r} \sum_{u=\lfloor r/4  \rfloor}^r \bP(\cC^u)\;.
\end{align*}
By further decomposing the probability of $\bP(\cC^u)$ in two parts depending on the value of the number of selections of arm $1$, we obtain the upper bound
\begin{align*}
\bP(\cZ^r \cap \overline{\cD}^r) & \leq  \frac{4}{r}\sum_{u=\lfloor r/4 \rfloor}^r \bP \left( N_1(u) \leq (\log u)^2 \right) + \frac{4}{r}\underbrace{\sum_{u=\lfloor r/4 \rfloor}^r \bP\left(\cC^u,  N_1(u) \geq (\log u)^2 \right)}_{B_r}\;.
\end{align*}
We now upper bound the quantity $B_r$ defined above by using Lemma \ref{concentration}. For each $a$, for any  $\omega_a$ such that $\omega_a \in (\mu_a, \mu_1)$, one can write
\begin{align*}
B_r &\leq \sum_{u=\lfloor r/4 \rfloor}^r \bP(\cC^u, N_1(u)\geq (\log \lfloor r/4 \rfloor)^2)\\
& \leq \sum_{k=2}^K \sum_{u=\lfloor r/4 \rfloor}^r \bP(Y_{k,N_1(u)-N_k(u):N_1(u)} > \bar Y_{1,N_1(u)}, N_1(u)\geq \log (\lfloor r/4 \rfloor)^2, N_k(u)>N_1(u)) \\
&\leq\sum_{k=2}^K \left( \frac{1}{1-e^{-\omega_k}} e^{- (\log \lfloor r/4 \rfloor)^2 \omega_k} + \frac{r}{1-e^{-\omega_k}} e^{-(\log \lfloor r/4 \rfloor)^2 \omega_k} \right)\;.
\end{align*}
%where the first inequality uses the fact that $N_1(u) \geq \log u^2 \Rightarrow N_1(u) \geq \log \left\lfloor \frac{s}{4} \right\rfloor^2$ when $u \geq \lfloor s/4 \rfloor$.
Choosing each $\omega_a$ such that $I_1(\omega_a)=I_a(\omega_a)$, we obtain: 
\begin{align*}\label{eq::bound_bis_C}
\begin{split}
\frac{4}{r}\sum_{r=8}^T  B_r & \leq \sum_{r=8}^T \sum_{k=2}^K \frac{4(r+1)}{r(1-e^{-\omega_k})}e^{-(\log \lfloor r/4 \rfloor)^2 \omega_k}\\
& \leq  \sum_{k=2}^K\sum_{r=8}^T \frac{6}{1-e^{-\omega_k}} e^{-(\log \lfloor r/4 \rfloor)^2 \omega_k},
\end{split}
\end{align*}
and for each $k$ the series in $r$ is convergent as for any constant $C$, $C\log(r) \leq (\log \lfloor r/4 \rfloor)^2$ for $r$ large enough. Hence, there exists some constant $D(\bm\nu)$ where $\bm\nu = (\nu_1,\dots,\nu_K)$ such that $\frac{4}{r}\sum_{r=8}^T  B_r \leq D(\bm\nu)$. It follows that 
\begin{align*}
\sum_{r=8}^{T}\bP(\cZ^r \cap \overline{\cD}^r) & \leq  \sum_{r=8}^{T}\frac{4}{r}\sum_{u=\lfloor r/4 \rfloor}^r \bP \left( N_1(u) \leq (\log u)^2 \right) + D(\bm\nu)\;.
\end{align*}
We now transform the double sum in the right-hand side into a simple sum by counting the number of times each term appears in the double sum:
$$\sum_{r=8}^T\frac{4}{r}\sum_{u=\lfloor r/4 \rfloor}^r \bP \left( N_1(u) \leq (\log u)^2 \right) = \sum_{r=8}^T \left( \sum_{t=1}^r \frac{4}{t} \ind(t \in [r, 4r]) \right) \bP(N_1(r)\leq (\log r)^2)\;.$$ 
Noting that $\sum_{t=1}^r \frac{4}{t} \ind(t \in [s, 4s]) \leq (4s-s+1)\times \frac{4}{s}\leq 16$, we finally obtain:
\begin{equation}\label{eq:termD}
\sum_{r=8}^{T}\bP(\cZ^r \cap \overline{\cD}^r)  \leq  16 \sum_{r=1}^{T} \bP\left(N_1(r) \leq (\log(r))^2\right) + D(\bm\nu). 
\end{equation}

Combining \eqref{eq::bound_B} and \eqref{eq:termD} yields 
\[\sum_{r=1}^{T} \bP\left(\cZ^r\right) \leq 16 \sum_{r=1}^{T} \bP\left(N_1(r) \leq (\log(r))^2\right) + D'_k(\bm\nu)\]
for some constant $D'_k(\bm\nu)$ that depends on $k$ and $\bm\nu$, which contributes to the final constant $C_k(\bm\nu,\epsilon)$ in Lemma~\ref{lem:dec}. Plugging this inequality in Equation~\eqref{eq:dec} concludes the proof of Lemma~\ref{lem:dec}. 

\tododo{Je ne remplace pas encore les unsolved reference et en reformule pas ce qu'on a écrit tant qu'on est pas sûr de complétement restate la preuve et de pas juste utiliser le lemme 4.1 du papier Neurips direct.}

